Teaching an Old LLM Secure Coding: Localized Preference Optimization on Distilled Preferences

LLM generated code often contains security issues. We address two key challenges in improving secure code generation. First, obtaining high quality training data covering a broad set of security issues is critical. To address this, we introduce a method for distilling a preference dataset of insecure and secure code pairs from frontier LLMs, along with a security reasoning that explains the issues and the fix. The key idea here is to make use of security knowledge sources to devise a systematic prompting strategy that ensures broad coverage. Second, aligning models to secure code requires focusing on localized regions of code. Direct preference optimization methods, like SimPO, are not designed to handle these localized differences and turn out to be ineffective. We address this with a new localized preference optimization algorithm that masks the security related tokens in both the winning (secure) and losing (insecure) responses. To prevent loss in code quality, we also add a regularizer. Evaluations show that both training on our dataset, DiSCo, and the new preference optimization algorithm, LPO, yield substantial reductions in code insecurity while also improving overall code quality. Code and dataset are available at https://github.com/StonyBrookNLP/disco-lpo.

==> latex/includes/macros.tex <==
\newcommand{\review}[1]{\smallskip\noindent\textit{\textit{#1}}\smallskip}
\newcommand{\reponse}[1]{\noindent{#1\\}}

%% Response text prefix
\newcommand{\respto}[1]{
    \fcolorbox{black}{black!15}{%
    \label{resp:#1}%
    \bf\scriptsize{\color{black}R{#1}}}\xspace%
}


%% Response text prefix
\newcommand{\bareresp}[1]{
    \fcolorbox{black}{black!15}{%
    \bf\scriptsize {\color{black}R{#1}}}\xspace%
}

% Cite responses
\newcommand{\citeresp}[1]{%
    {(see }\fcolorbox{black}{black!15}{%
    \bf\scriptsize R{#1}}~{{on page \pageref{resp:#1})}}%
}\xspace%

\newenvironment{response}
{\color{blue}}
{\color{black}}


\newcommand{\errorcode}[1]{
    \colorbox{redish}{\bf {\small \texttt{#1}}}
}


\newcommand{\MSH}[1]{{\todo{{\color{blue} #1} - {\small MSH}}}}
\newcommand{\NB}[1]{{\todo{{\color{violet} #1} - {\small NB}}}}
\newcommand{\SKK}[1]{{\todo{{\color{purple} #1} - {\small SKK}}}}
\newcommand{\SC}[1]{{\todo{{\color{orange} #1} - {\small SC}}}}


\newcommand{\checkme}[1]{{\color{red}#1}}

\newcommand{\cross}{\ding{55}}
\newcommand{\tick}{\ding{51}}



\newtcbox{\inlinebox}[1][]{enhanced,
 box align=base,
 nobeforeafter,
 colback=blueish,
 size=small,
 left=0pt,
 right=0pt,
 boxsep=2pt,
 #1}
 

\newcommand{\highlight}[1]{%
{\footnotesize%
\inlinebox{#1}%
}}

\newcommand{\sdata}{
{$B2F_{s}$}\xspace
}
\newcommand{\mdata}{
{$B2F_{m}$}\xspace
}

\newcommand{\ud}{\textbf{\_}}

\newcommand{\lessons}[1]{
    \footnotesize
    \begin{lesson}
        \tick~#1
    \end{lesson}
}

\newcommand{\RQrepeat}[2]{%
    {\footnotesize
    \begin{question}
        \noindent{\textbf{\hyperref[rq-#1]{RQ#1.}~#2}}
    \end{question}}
}

\newcommand{\RQ}[2]{%
    {
    \footnotesize
    \vspace{.3em}
    \begin{question}
        \label{rq-#1}
        \noindent\textbf{{RQ{#1}.~#2}}
    \end{question}}
}

\newcommand{\RS}[2]{%
    {
    \begin{result}
        \textbf{\hyperref[rq-#1]{Result {#1}}:~}{{#2}}%
    \end{result}}
}

\renewcommand{\cref}[1]{\Cref{#1}}



\newcommand{\para}[1]{
    \smallskip
    
    \underline{\it #1.}
}

\newcommand{\motivation}{
    \para{Motivation}
}

\newcommand{\experiment}{
    \para{Experimental Setup}
}

\newcommand{\resultsec}{
    \para{Results}
}

\newcommand{\analysis}{
    \para{Analysis}
}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.,}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.,}}\xspace}
\newcommand{\st}{\hbox{\emph{s.t.,}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace}
\newcommand{\vs}{\hbox{\emph{v.s.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}


\newtheorem{theorem}{Theorem}[section]
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\varname}[1]{{\small\texttt{#1}}\xspace}
%\newcommand{\tom}[1]{{\color{red} Tom: #1}\xspace}
\newcommand{\ch}[1]{{\color{black} #1}\xspace}
%\newcommand{\tableshrink}[1]{\vspace{-0.25in}}




\def\wv{\superscript{\S}}
\def\wu{$^{\dag}$}
\def\wg{\superscript{\ddag}}
\def\wn{$^{\natural}$}

\definecolor{gray50}{gray}{.5}
\definecolor{gray40}{gray}{.6}
\definecolor{gray30}{gray}{.7}
\definecolor{gray20}{gray}{.8}
\definecolor{gray10}{gray}{.9}
\definecolor{gray05}{gray}{.95}
\definecolor{gray01}{gray}{.97}

\newlength\Linewidth
\def\findlength{\setlength\Linewidth\linewidth
\addtolength\Linewidth{-4\fboxrule}
\addtolength\Linewidth{-3\fboxsep}
}
\newenvironment{examplebox}{\par\begingroup
  \setlength{\fboxsep}{3pt}\findlength
  \setbox0=\vbox\bgroup\noindent
  \hsize=0.90\linewidth
  \begin{minipage}{0.90\linewidth}\normalsize}
    {\end{minipage}\egroup
%    \vspace{6pt}
    \textcolor{gray20}{\fboxsep1.2pt\fbox
     {\fboxsep5pt\colorbox{gray05}{\normalcolor\box0}}}
%    \endgroup\par\addvspace{6pt minus 3pt}\noindent
    \endgroup\par\noindent
    \normalcolor\ignorespacesafterend}
\let\Examplebox\examplebox
\let\endExamplebox\endexamplebox

%-------------------------------------------------------------------------------------------
% Research Questions and Results
%
\newcounter{RQCounter}
\newcounter{RQACounter}

 %Pass in label for rq, then rq
%

% \newcommand{\RQ}[2]{%
% \refstepcounter{RQCounter} \label{#1}
%  \begin{center}	
%   \begin{examplebox}
%   \textbf{RQ\arabic{RQCounter}.}#2
%   \end{examplebox}	 
%  \end{center}
% }

% --- Material style Result Box ---
% \usepackage[framemethod=tikz]{mdframed}
\usetikzlibrary{shadows}
\usepackage{graphics}
\newmdenv[
    tikzsetting= {fill=blueish},
    skipabove=0.33em,
    skipbelow=0.33em,
    linewidth=1pt,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
    linecolor=gray95,
    roundcorner=2pt, 
    shadow=true,
    shadowsize=4pt,
    shadowcolor=gray95
]{questionbox}

\newmdenv[
    tikzsetting= {fill=greenish},
    skipabove=0.33em,
    skipbelow=0.33em,
    linewidth=1pt,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
    linecolor=gray95,
    roundcorner=2pt, 
    shadow=true,
    shadowsize=4pt,
    shadowcolor=gray95
]{answerbox}

\newmdenv[
    skipabove=0.33em,
    skipbelow=0.33em,
    innerleftmargin=4pt,
    innerrightmargin=4pt,
    innertopmargin=2pt,
    innerbottommargin=2pt,
]{lessonbox}

\usepackage{tikz}
\newcommand*\circled[1]{
    % \vspace{-1mm}
    \hspace{-.5em}
    \tikz{
        \draw[fill=none, draw=#1, thick] (0,-0.1) circle (1.3mm);
        \draw[->, thick, #1] (-0.07,-0.1) -- (.10,-0.1); 
    } 
    \hspace{-.6em}
}

\newcommand*\sre{
    % \hspace{-.5em}
    \circled{step1}\xspace
}

\newcommand*\spremise{
    \circled{step2}\xspace
}

\newcommand*\sprompt{
    \circled{step3}\xspace
}

\newcommand*\sgen{
    \circled{step4}\xspace
}

\newcommand*\sver{
    \circled{step5}\xspace
}




%\captionsetup{belowskip=3pt,aboveskip=3pt} % space between caption and content
\renewcommand\tabularxcolumn[1]{m{#1}} % tabularx align vertically
%\newcolumntype{s}{>{\centering \arraybackslash \hsize=.5\hsize}X}  % 

\newenvironment{lesson}
{
    \begin{lessonbox}
}
{\end{lessonbox}}




\newenvironment{result}
{\begin{answerbox}}
{\end{answerbox}}

\newenvironment{question}
{\begin{questionbox}}
{\end{questionbox}}



\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc

\lstdefinestyle{basejava}{
  language=java,
  showstringspaces=false,
  basicstyle=\scriptsize\ttfamily,
  keywordstyle=\bfseries\color{javapurple},
  commentstyle=\itshape\blue,
  identifierstyle=\blue,
  frame=none,
  backgroundcolor=\color{white},
}


\lstdefinestyle{CustomJava}{
  belowcaptionskip=\baselineskip,
  breaklines=true,
  xleftmargin=\parindent,
  language=java,
  showstringspaces=false,
  basicstyle=\scriptsize\ttfamily,
  keywordstyle=\bfseries\color{javapurple},
  commentstyle=\itshape\blue,
  identifierstyle=\blue,
  belowskip=1pt,
  frame=shadowbox,
  backgroundcolor=\color{gray01},
  gobble=0
}

\lstset{escapechar=@,style=customjava}

\newtcblisting{mylisting}[2][]{
    %arc=0pt, outer arc=0pt,
    %width=\columnwidth,
    arc=3mm,
    listing only, 
    listing style=codit,
    title=#2,
    #1
    }    

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}





==> latex/includes/pygments.tex <==
\newcommand\at{@}
\newcommand\lb{[}
\newcommand\rb{]}
\newcommand\Red[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{#1}}}
\newcommand\red[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\grayline[1]{\textcolor[rgb]{0.4,0.4,0.4}{{#1}}}
\newcommand\gray[1]{\colorbox[rgb]{0.8,0.8,0.8}{{#1}}}
\newcommand\brown[1]{\textcolor[rgb]{0.55,0.27,0.07}{#1}}
\newcommand\orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{\textbf{#1}}}
\newcommand\Orange[1]{\textcolor[rgb]{1.00,0.55,0.30}{{#1*}}}
%\newcommand\green[1]{\textcolor[rgb]{0.42,0.56,0.14}{#1}}
\newcommand\lime[1]{\textcolor[rgb]{0.13,0.55,0.13}{{#1}}}
\newcommand\blue[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\blued[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1$\dag$}}}
\newcommand\ColorLine[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}
\newcommand\javagreen[1]{\textcolor[rgb]{0.25,0.5,0.35}{{#1}}}
\newcommand\javadocblue[1]{\textcolor[rgb]{0.25,0.35,0.75}{{#1}}}
\newcommand\dkgreen[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\green[1]{\textcolor[rgb]{0.0,0.6,0}{#1}}
\newcommand\Green[1]{\textcolor[rgb]{0.0,0.6,0}{\textbf{#1}}}
\newcommand\Greenul[1]{\textcolor[rgb]{0.0,0.6,0}{{#1}}}
\newcommand\mauve[1]{\textcolor[rgb]{0.58,0.0,0.82}{{#1}}}
\newcommand\yellow[1]{\textcolor[rgb]{1,0.9,0.5}{{\bf #1}}}
\newcommand\lblue[1]{\colorbox[rgb]{0.87,1,1}{{#1}}}

\newcommand\PYbg[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbf[1]{\textcolor[rgb]{0.73,0.40,0.53}{\textbf{#1}}}
\newcommand\PYbe[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYbd[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYbc[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYbb[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYba[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaJ[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaK[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaH[1]{\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{#1}}
\newcommand\PYaI[1]{\textcolor[rgb]{0.69,0.00,0.25}{#1}}
\newcommand\PYaN[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaO[1]{\textcolor[rgb]{0.00,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaL[1]{\textcolor[rgb]{0.73,0.73,0.73}{#1}}
\newcommand\PYaM[1]{\textcolor[rgb]{0.74,0.48,0.00}{#1}}
\newcommand\PYaB[1]{\textcolor[rgb]{0.00,0.25,0.82}{#1}}
\newcommand\PYaC[1]{\textcolor[rgb]{0.67,0.13,1.00}{#1}}
\newcommand\PYaA[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaF[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand\PYaG[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaD[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaE[1]{\textcolor[rgb]{0.63,0.00,0.00}{#1}}
\newcommand\PYaZ[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaX[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaY[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaR[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYaS[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYaP[1]{\textcolor[rgb]{0.49,0.56,0.16}{#1}}
\newcommand\PYaQ[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaV[1]{\textcolor[rgb]{0.00,0.00,1.00}{\textbf{#1}}}
\newcommand\PYaW[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaT[1]{\textcolor[rgb]{0.50,0.00,0.50}{\textbf{#1}}}
\newcommand\PYaU[1]{\textcolor[rgb]{0.82,0.25,0.23}{\textbf{#1}}}
\newcommand\PYaj[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYak[1]{\textcolor[rgb]{0.73,0.40,0.53}{#1}}
\newcommand\PYah[1]{\textcolor[rgb]{0.63,0.63,0.00}{#1}}
\newcommand\PYai[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYan[1]{\textcolor[rgb]{0.67,0.13,1.00}{\textbf{#1}}}
\newcommand\PYao[1]{\textcolor[rgb]{0.73,0.40,0.13}{\textbf{#1}}}
\newcommand\PYal[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYam[1]{\textbf{#1}}
\newcommand\PYab[1]{\textit{#1}}
\newcommand\PYac[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYaa[1]{\textcolor[rgb]{0.50,0.50,0.50}{#1}}
\newcommand\PYaf[1]{\textcolor[rgb]{0.25,0.50,0.50}{\textit{#1}}}
\newcommand\PYag[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYad[1]{\textcolor[rgb]{0.73,0.13,0.13}{#1}}
\newcommand\PYae[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYaz[1]{\textcolor[rgb]{0.00,0.63,0.00}{#1}}
\newcommand\PYax[1]{\textcolor[rgb]{0.60,0.60,0.60}{\textbf{#1}}}
\newcommand\PYay[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYar[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYas[1]{\textcolor[rgb]{0.73,0.13,0.13}{\textit{#1}}}
\newcommand\PYap[1]{\textcolor[rgb]{0.00,0.50,0.00}{#1}}
\newcommand\PYaq[1]{\textcolor[rgb]{0.53,0.00,0.00}{#1}}
\newcommand\PYav[1]{\textcolor[rgb]{0.00,0.50,0.00}{\textbf{#1}}}
\newcommand\PYaw[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}
\newcommand\PYat[1]{\textcolor[rgb]{0.10,0.09,0.49}{#1}}
\newcommand\PYau[1]{\textcolor[rgb]{0.40,0.40,0.40}{#1}}

\newcommand\merun[1]{\textcolor[rgb]{0.45,0.0,0.0}{#1}}
\newcommand\purple[1]{\textcolor[rgb]{0.22,0.0,0.44}{#1}}
\newcommand\javaKeyWord[1]{\textcolor[rgb]{0.38,0.03,0.58}{\tt \textbf{#1}}}

\definecolor{blueish}{RGB}{252, 252, 255}
\definecolor{greenish}{RGB}{252, 255, 252}
\definecolor{redish}{RGB}{255, 250, 250}


% ---- Grays ----
\definecolor{gray05}{gray}{0.95}
\definecolor{gray08}{gray}{0.92}
\definecolor{gray10}{gray}{0.90}
\definecolor{gray12}{gray}{0.88}
\definecolor{gray15}{gray}{0.85}
\definecolor{gray18}{gray}{0.82}
\definecolor{gray20}{gray}{0.80}
\definecolor{gray25}{gray}{0.75}
\definecolor{gray30}{gray}{0.70}
\definecolor{gray35}{gray}{0.65}
\definecolor{gray40}{gray}{0.60}
\definecolor{gray45}{gray}{0.55}
\definecolor{gray50}{gray}{0.50}
\definecolor{gray55}{gray}{0.45}
\definecolor{gray60}{gray}{0.40}
\definecolor{gray65}{gray}{0.35}
\definecolor{gray70}{gray}{0.30}
\definecolor{gray75}{gray}{0.25}
\definecolor{gray80}{gray}{0.20}
\definecolor{gray85}{gray}{0.15}
\definecolor{gray90}{gray}{0.10}
\definecolor{gray95}{gray}{0.05}

\definecolor{fstarid}{rgb}{0.28,0.07,0.07}

\definecolor{addition}{rgb}{0,0.1,0.5}
\definecolor{dkblue}{rgb}{0,0.0,0.7}
\definecolor{dkgreen}{rgb}{0,0.4,0}
\definecolor{dkred}{rgb}{0.6,0,0}
\definecolor{dkpurple}{rgb}{0.55,0,0.75}
\definecolor{purple}{rgb}{0.69,0,.87}
\definecolor{olive}{rgb}{0.4, 0.4, 0.0}
\definecolor{teal}{rgb}{0.0,0.4,0.4}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{gray}{rgb}{0.5, 0.5, 0.5}
\definecolor{dkgrey}{rgb}{0.2, 0.2, 0.2}
\definecolor{lilac}{rgb}{0.70, 0.04, 0.08}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}

\definecolor{step1}{HTML}{CC0066}
\definecolor{step2}{HTML}{CC6600}
\definecolor{step3}{HTML}{440077}
\definecolor{step4}{HTML}{007700}
\definecolor{step5}{HTML}{0000FF}


==> latex/scratch-pad.tex <==
\begin{figure}[!ht]
  \centering
\includegraphics[width=1.0\columnwidth]{latex/diagrams/intro.pdf}
  %
  \caption{
  %\nb{Fix this caption, we no longer use slposr}
  \small
  \textbf{\Task{} using \dataset{} and \alignment{}}: In this example, untuned LLMs generate insecure \textcolor{red}{\texttt{yaml.load()}} due to lack of knowledge about code security. Our method solves this by tuning LLMs on synthesized  data \dataset{} using preference algorithm \alignment{},so that LLMs knows to use the secure definition \textcolor{teal}{\texttt{yaml.safe\_load()}}. 
  % LLMs do not always have adequate knowledge about code security. For instance, in this code completion task, the LLM generates \textcolor{red}{\texttt{yaml.load()}} which is an unsafe function. \name overcomes this issue by training LLMs to learn secure coding practises from synthetic datasets distilled from frontier models using a combination of security reasoning and localized preference optimization algorithms designed for the task. As a result, the trained LLM is able to do the same code completion task using \textcolor{teal}{\texttt{yaml.safe\_load()}).}, a more secure definition doing the same functionality. 
  }
  \vspace{-2em}
  \label{Fig:intro}
\end{figure}



==> latex/sections/methodology.tex <==
%\section{Methodology}
%Addressing the aforementioned challenges faced when aligning models towards secure code generation, we design a strategy combining synthetic data distillation \cite{} and preference optimization \cite{} called \textit{Synthetic Localized Preference Optimization} or \name in short. \name uses prompt engineering to distill synthetic data from larger powerful LLMs. This data is then used to align models using preference optimization algorithms tailored for the task.





%Equation for RLHF
%Equation for Preference Optimization


% To create our dataset, we choose the path of knowledge distillation using more powerful LLMs. The technique involves prompting larger more powerful LLMs to generate (input,output) data pairs which can then be used for aligning smaller sized LLMs. This is quite a popular method used nowadays to generate synthetic data. For example, \sh{add a bunch of paper that generates synthetic data using LLMs}. 

\section{Synthetic Distillation}

\nb{First, restate your goal of deriving synthetic data from an LLM. Here you can support this by pointing to other works that have done so for other problems, perhaps even for code related things. Then, explain why a simple direct prompting is problematic using one example (or more as needed). The issues are (i) LLM safeguards often block generation of code with security issues (say you have observed this and if you have any papers refer to it), (ii) misalignment of the different parts of the data (insecure code, the secure code, and the reasoning), (ii) hallucination of security vulnerabilities, (iii) inability to fix the security issues directly during generation in one go or introducing other security issues. Last, at a high-level simply state the main steps in your pipeline and how they will address these issues.}


In order to solve the data challenge, we follow the path of synthetic data generation using LLM knowledge distillation. It means that we prompt larger, more powerful LLMs with prompts in order to generate synthetic data rows. This is then used to train the smaller LMs. This knowledge distillation paradigm has shown to be effective for a variety of tasks where annotating datasets has been an issue like this\cite{} and that \cite{}. Many LLMs are being trained via knowledge distillation from larger LLM or even from themselves \cite{}. In order to effectively generate synthetic data using LLMs for alignment, we need to engineer effective prompts such that LLM follows the instructions properly and does not hallucinate. Else, the data generated will be of lower quality and will not help in training the model. As such, for our synthetic data generation purposes, we develop a prompting pipeline where we first extract knowledge about code security that exist out there in the form of rules and descriptions. These are then used to generate fine-grained prompts using templates in order to effectively prompt the model . As a result, the generated data adheres better to the prompt and is more effective. For further fine-grained data, we introduce a refine step where the data generated, specifically the secure code, is passed through a verifier and refined based on security issues prevalent in it.




Our synthetic data generation process consists of a pipeline with the following component: knowledge aggregation, templating, distillation, feedback \& refinement.

\paragraph{Knowledge Aggregation} 
\nb{Take care of redundancy. You will have said some of the main steps (e.g. generating synthetic data) already. There is no need to repeat them here.}
\nb{What are the key properties of security vulnerabilities that are needed in generating and avoid code with security issues? Mention them here and then say how you can derive these using the resources you mention below.}
LLMs can be prompted to generate synthetic datasets. However, LLMs tend to hallucinate\cite{}. One way of tackling this is to augment LLMs prompts with knowledge about the target domain. Hence, for distilling useful synthetic data from LLMs, we have to enhance the prompts via knowledge from security domains.
Such knowledge have been accumulated by security experts and is scattered across various open-source hubs. They exist in many different forms: rules in existing security analysis tools; descriptions on open-source information databases etc. Based on these multiple sources of information, we boil to the following three sources: CodeQL, Bandit \& Common Weakness Enumeration (CWE) database. CodeQL is a semantic security analysis tool and Bandit is a static security analyzer. Both these tools have enumerations of common code  security issues that these analyzers can detect. The third source, CWE, is a database of the common code securities that can exist across code, maintained by the Mitre Corporation. We extract the rules used by CodeQL and Bandit for detecting vulnerabilities from their documentation and the descriptions of vulnerabilities from the CWE website. In this way, we gather $534$ tuples of (id,title,summary) where title is the name of the issue, summary contains the description and id corresponds to the CWE-ID of the issue.
To further enhance, our prompts, we search through the Python Package Index (pypi), a database of open-source Python project repositories, to extract the names of topmost libraries. Our search was limited to libraries from the networking and cybersecurity domains as these domains are the ones that contain the most security issues. 
\nb{Move this to a dataset statistics table. The synthetic dataset should be summarized compactly in such a table.}
In this way, we gather $75$ different names of modules. We are able to procure $534$ rows of information regarding different security issues and $75$ different Python module names where such issues can exist. 

\paragraph{Prompt Templating}
\nb{First state what it is that you want to achieve and then say how you achieve this. Something like: 
We want the generated code to be x and y. We achieve by using two templates.}
Utilizing this extracted information, we construct two sets of prompts based on two different prompt templates. The first prompt template uses the \textit{title} and \textit{description} from each row of security issue information and we get around $534$
different prompts. The second prompt template uses a combination of the \textit{(title,description)} columns from the security issue information dataset and the module names to create around $534 \times 75 =40050$ unique prompts. We sample around $9500$ different prompts from this set. In this way, we have around $10534$ different prompts for distillation. The prompt templates are given in the Appendix.

\paragraph{Distillation} \nb{We use these prompts in the following process to obtain the distillation data. }

%After formulating around $\approx 10000$ different prompts, we prompt a large and powerful LLM to generate our synthetic data. 

We use \texttt{GPT-4o} \cite{} as our code generation model, since it has been shown to generate high quality code in many domains\nb{cite}. \nb{The model is prompted to generate the following in a sequence: (i) }

is designed to generate the vulnerable code first followed by the secure version of the code. Then the LLM is asked to generate the natural language summary that be used to describe either of the codes. The summary is designed in such a way that it can be used as an instruction for instruction tuning LLMs. The reason for this design choice is that we observed that if asked to generate the natural language summary before the vulnerable code, then the model does not follow the instructions in the prompt effectively, resulting in disjoints between elements in the (summary, vulnerable code, secure code), thereby reducing the effectiveness of the dataset.

\paragraph{Feedback \& Refinement} After data generation using the previous two steps, we observed that a substantial portion of the `secure code' in our dataset (37\%) still contained security vulnerabilities. \nb{Some of these were cases where the LLM did not fix the original issue in the insecure code. Others are where the LLM ended up introducing other vulnerabilities not relevant to the original security vulernability mentioned in the prompt. For example, [COMPLETE THIS].} 

To address this, we introduce a \textbf{refinement} step. First, we run the open-source security analyzers, CodeQL and Bandit, on the generated secure code to identify security issues and relevant feedback on fixing the issues. Then, we design a refine prompt template (template is provided in the Appendix) that adds the identified issues and feedback, if any, to each piece of secure code. We then feed this refine prompt to \texttt{GPT-4o} to fix the identified issue. \nb{Fix the following description if you want things to be more formally stated.} The final code, secure code++, is then appended to the (instruction, insecure code, secure code) dataset. 

\paragraph{Final Dataset} \nb{Instead of the content below, use this space to provide overall statistics of the dataset and maybe some information about the coverage of the security issues in your dataset.}

Using the process above, we generate a dataset of (natural language summary, insecure code, secure code, secure code ++) tuples. This dataset is then formatted to the structure of (natural language summary, insecure code, secure code) where secure code is replaced by secure code++ if the data point was refined. This dataset is then divided into train, validation and test datasets for alignment. This is described in the next section
Figure \ref{Fig:synthetic_data} provides a visualization of the whole synthetic data generation pipeline.








\begin{figure*}[!ht]
  \centering
\includegraphics[width=1.0\textwidth]{latex/diagrams/synthetic_data.pdf}
  %
  \caption{\small{\textbf{Synthetic Data Creation Pipeline}:
  }
  }
  \label{Fig:synthetic_data}
\end{figure*}




\section{Localized Preference Optimization}

For the challenge of alignment, we design a novel alingnment algorithm based on preference optimization. Preference optimization (PO) algorithms, synonymous with Direct Preference Optimization algorithms, are a set of LLM optimization algorithms based on reinforcement learning via human feedback (RLHF). RLHF works by first training a reward model from a preference data of samples rated by humans. Then the actual model is trained by having the reward model rank and rate generations and using that as loss signals for backpropagation. Whereas RLHF requires a reward model in order to provide signal for training, PO does not have such requirement. They skip the process of reward models altogether by introducing a loss function that learns the reward function directly from the preference data. This is usually done by optimizing by having a preference data of positive (higher ranked) and negative (lower ranked) sample and then learning a loss that has a higher log-likelihood of generating the postive sample than the negative one. We choose this paradigm of learning as it has shown effectiveness for a range of LLM tasks like this \cite{} and that{}. Also, preference optimization, being a loss function that learns the contrast between generations, is ideal for secure code generation task as it involves differentiating between positive and negative. While a slew of PO algorithms exist across the domain, we choose SimPO as it has shown great promise in recent times. We further enhance this preference optimization algorithm by introducing an extra element that makes the model focus on the security tokens, inspired by the needle-in-the-haystack problem of secure coding. We call this \textit{LPO} and do this by introducing masks to the PO algorithms. Another issue that occurs in secure code generation tasks is \textit{code degeneralization}. To address this in PO, we further modify \textit{LPO} to introduce \textbf{LPO-reg}. \textit{LPO-reg} tries to reduce the code degeneralizaiton by making sure the log-likelihood of the non-security tokens in code is not reduced as a result of the PO.

After generating the synthetic dataset of (instructions,secure code,insecure code), we align our models using our \textit{localized preference optimization} technique.

As common across many works, our first step for aligning LLMs using preference optimization algorithms is to perform supervised finetuning. The supervised fine-tuning step involves training the model to generate positive sample conditioned upon the prompt using language modelling loss. In our case, it is to train the model to generate the secure code given the natural language instruction:

%Equation for SFT

From training this model, we get the $\Pi_{sft}$ model. This model itself is then further training using the preference optimization algorithm. As mentioned, we choose the Simple Preference Optimization (SimPO) algorithm as our base preference optimization algorithm:

%Equation for SimPO

This preference optimization algorithms work by forcing the model to learn that the average log probability of the positive sample should be higher than the negative sample given the same prompt, thereby encouraging the model to generate the positive sample in this context. The average log probability is calculated by taking into account the probability of the whole sequence, including tokens non-relevant to the security issue of the code and that exist in both pieces of code.

Inspired by the concept of ``needle in the haystack'' that exist in the secure coding problem spaces, we modify the SimPO algorithm by introducing two masks: a positive sample mask and a negative sample mask. The mask is a zero-one vector that determines what portion of the each sample is relevant to its security. This is determined by identifying the differing portions between the two pieces of code: tokens unique to the insecure code are the ones that contribute to security issues whereas tokens unique to the secure code are the ones that makes it more secure. We can easily do this via libraries such as the Python difflib library. In this way, two masks, $m_{+}$ and $m_{-}$ are included. These respective masks are then used to take into account the log probabilites of only the security relevant tokens by modifying the loss as follows:

%Updated SimPO loss function

\paragraph{Code Degeneralization} Previous works on secure code generation like \citep{sven} and \citep{safecoder} show that training LLMs for secure code generation adeversely affects the models ability general coding abilities. Preference optimization algorithms have also been observed to possess the \textit{degeneration} issue akin to many reinforcement learning algorithms. This problem is that model optimizes so much to the reward model/mechanism that it loses it's generalization capability, thereby generating garbage that only makes the reward model happy but is not coherent with the other loss functions like language modelling. Based on these intuitions, we further modify the LPO algorithm to design LPO-reg. Our assumption for code degeneralization in our setting is that the model focusses so much on the security tokens that it only learns about them and ignores about the surrounding context, whether they are coherent or not. In such usecases, it is imperative that the model also does not lose out on its ability to generate this context for the positive sample. Taking this into account, we insert a regularization element in the loss function that makes sure that the model does not forget the language modelling loss of the surrounding context for the positive sample. We first calculate the anti-mask of the positive sample and then multiply it with the log probabilities of the postive sample. This is then added to the loss function to prevent the model from losing its language modelling capabilities:

%Equation for LPO-reg






\begin{figure*}[!ht]
  \centering
\includegraphics[width=1.0\textwidth]{latex/diagrams/PLO.pdf}
  %
  \caption{\small{\textbf{Synthetic Data Creation Pipeline}:
  }
  }
  \label{Fig:intro}
\end{figure*}





% \sh{I am dumping ideas on this section. I will have it finalized before Saturday for reviewing.}
% In order to solve the \textit{secure code generation} task, we need to teach models about the security issues pertaining to code. This requires two important things: datasets \& alignment techniques. 

% \subsection{Secure Training Datasets} To train LLMs to generate secure code, we need to teach them to differentiate between secure code and insecure code. In order to do so, we need to obtain datasets containing a code with with a security issue and the corresponding code with the issue resolved. Unfortunately, obtaining such datasets for training LLMs is not easy. Manual curation of such datasets are difficult as you need domain expertise to understand security vulnerabilities. Also, writing code with specific vulnerabilities using humans is expensive both in terms of cost of expertise as well as time. The next best alternative lies in using automatic methods or open-source environments. The general pipeline for gathering such datasets involve accumulating insecure code and the corresponding fixed version from open-source databases like GitHub. This is usually done via keyword matching to see if the commits mention security issues. Some works perform further fine-grained selection using automatic seccurity analysis tools like CodeQL \cite{}. Other works extract data from security enumerated databases like Common Vulnerabilites and Exposures (CVEs) as annotations gathered from such sites are more reliable. Many popular security detection datasets like BigVul \cite{} and CVEFixes dataset \cite{} have been gathered in this way. However, datasets gathered in this way are not always optimal for training lLMs for secure code generation. For instance, automatically selecting and labelling data by matching security based keywords of the commits can lead to inaccurate labels as commits may not point to securitu issues, resolve the issues, ro resolve it using ad-hoc manner. Such datasets also have low coverage as they are gathered from just a small set of projects and/or do not cover a lot of CWEs. Furthermore, automatically gathered datasets that go through  multiple layers of checks and heuristics, like the ones proposed in \citep{sven} or \citep{safecoder}, create very small amount of data ( usually in the 100s) which is very small for properly training LLMs. Furthermore, these datasets, while being representative of real-world coding practices as they come from open-source repositories, do not possess strong signals that help models learn the rules of secure coding, i.e., they are not curriculum \sh{Does this make sense. Write it better.}.

% \subsection{Secure Code Generation} The second important aspect of the \textit{secure code generation} task is to align LLMs towards secure code generation using these datasets, i.e, train them. This is a new area of research that is gaining traction. One way of doing is to pre-train LLMs using code data that has already been vetted for security issues using security analyzers. For example, \citep{Starcoder} trained the Starcoder model using such cleaned pre-training data and was shown to perform much better on the \citep{asleep_at_the_keyboard} secure code generation benchmark compared to other code foundation models. Another way of aligning is to directly perform supervised fine-tuning \cite{} on the secure code from the datasets. However, there is an issue to this type of training: models have no ways of knowing what constitutes the security issue. \citep{sven} is one of the first papers to identify this issue in secure code generation task. They propose a multi-component loss function that makes the model learn to focus on the security portion of the code using masks while learning the difference between secure and insecure code via contrastive learning. They also incorporate a KL-divergence loss in order to reduce the loss in code generation capabilities as models are trained for secure coding. \citep{safecoder} incorporates this same idea of focussing via masking by instruction tuning LLMs with a SFT loss function that masks out everything except those tokens relevant to the security of the code. While these ideas have been shown to learn effective secure code generation, no work as of now has embodied the concept of reinforcement learning\cite{} for secure code generation, in particular the \textit{preference optimization} (PO) paradigm. Direct preference optimization \cite{} and its variants like Simple Preference Optimization \cite{} have shown significant performance gains for LLMs on aligning models towards generations ranked better by humans. PO does this by teaching the model to contrast between preferred or higher ranked outputs with lower ranked generations. This type of discrimination is also essential for learning secure code generation as models should be able to prefer generating the secure code instead of the insecure ones. Hence, PO algorithms should be natural choices for this task. However, they have not been applied to this task as of now as per our knowledge. 



==> latex/sections/results_and_analysis_old.tex <==
\section{Results \& Analysis}

\subsection{Main Results}

\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}  % Increase row spacing
    \begin{tabular}{l l *{9}{c}}  % Center-align numeric columns
     \toprule
     \multirow{3}{*}{\textbf{Models}} & \multicolumn{10}{c}{\textbf{Datasets}} \\
     \cmidrule(lr){2-11}
     & \multicolumn{2}{c}{SecEval} & \multicolumn{2}{c}{Asleep} & \multicolumn{2}{c}{LLMSecEval} & \multicolumn{2}{c}{Synth.} & HumEvalX & MBPP\\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-10}\cmidrule(lr){11-11}
     & FS & BE & FS & BE & FS & BE & FS & BE & Pass@1 & Pass@1\\
     \midrule
    \textbf{CodeLlama}  &  &  &  &  &  &  &  &  &  & \\
    \hspace{0.5em}Base      & 54.02 & 83.93 & 92.00 & 172.00 & -- & -- & -- & -- 
    & 29.27 
    & -- \\
    \hspace{0.5em}SFT       & 18.82 & 30.76 & 89.23 & 145.38 & -- & -- & -- & -- 
    & 36.59 
    & -- \\
    \hspace{0.5em}PO        & 29.24 & 47.06 & 90.00 & 151.54 & -- & -- & -- & -- 
    & 34.15 
    & -- \\
    \hspace{0.5em}LPO-reg   & 14.71 & 26.99 & 51.18 & 70.87 & -- & -- & -- & -- 
    & 36.59 
    & -- \\
     \midrule
     \textbf{Starcoder-2}  &  &  &  &  &  &  &  &  &  & \\
    \hspace{0.5em}Base      & 55.84 & 86.94 & -- & -- & -- & -- & -- & -- 
    & 31.71 
    & -- \\
    \hspace{0.5em}SFT       & 27.06 & 44.71 & -- & -- & -- & -- & -- & -- 
    & 39.02
    & -- \\
    \hspace{0.5em}PO        & 26.14 & 41.32 & -- & -- & -- & -- & -- & -- 
    & 40.24
    & -- \\
    \hspace{0.5em}LPO-reg   & 16.41 & 21.54 & -- & -- & -- & -- & -- & -- 
    & 40.85
    & -- \\
     \midrule
     \textbf{Mistral}  &  &  &  &  &  &  &  &  &  & \\
    \hspace{0.5em}Base      & 52.99 & 83.98 & -- & -- & -- & -- & -- & -- 
    & 24.39
    & -- \\
    \hspace{0.5em}SFT       & 27.97 & 38.99 & -- & -- & -- & -- & -- & -- 
    & 37.80 
    & -- \\
    \hspace{0.5em}PO        & 5.86 & 8.54 & -- & -- & -- & -- & -- & -- 
    & 37.80
    & -- \\
    \hspace{0.5em}LPO-reg   & 2.33 & 3.49 & -- & -- & -- & -- & -- & -- 
    & 31.71
    & -- \\
     \midrule
     \textbf{Phi-2}  &  &  &  &  &  &  &  &  &  & \\
    \hspace{0.5em}Base      & 52.55 & 87.52 & -- & -- & -- & -- & -- & -- 
    & 50.00
    & -- \\
    \hspace{0.5em}SFT       & 23.44 & 32.81 & -- & -- & -- & -- & -- & -- 
    & 53.05 
    & -- \\
    \hspace{0.5em}PO        & 24.79 & 35.04 & -- & -- & -- & -- & -- & -- 
    & 53.66
    & -- \\
    \hspace{0.5em}LPO-reg   & 19.20 & 28.03 & -- & -- & -- & -- & -- & -- 
    & 53.05
    & -- \\
     \bottomrule  % Changed from \midrule to \bottomrule for the last line
    \end{tabular}
    \caption{Overall performance of various LLMs trained on our dataset. FL and BL denote Function-Level and Block-Level evaluations respectively.}
    \label{tab:main_table}
\end{table*}





\subsection{Comparison with Other Security Tuning Methods}


\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l *{3}{c}}
     \toprule
     \multirow{3}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{Datasets}} \\
     \cmidrule(lr){2-4}
     & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX} \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
     & FS & BL & Pass@1 \\
     \midrule
     \textbf{Phi-2} &  &  &  \\
     \hspace{0.5em}SVEN & 55.77 & 86.71 & 28.05 \\
     \hspace{0.5em}SafeCoder & 23.54 & 27.57 & 29.88 \\
     \hspace{0.5em}\textbf{LPO-Reg} & 19.20 & 28.03 & 53.05 \\
     \midrule
     \textbf{CodeLlama} & & &  \\
     \hspace{0.5em}SafeCoder & 11.66 & 16.20 & 15.24 \\
     \hspace{0.5em}\textbf{LPO-Reg} & 14.71 & 26.99 & 36.59 \\
     \midrule
     \textbf{Mistral} & & &  \\
     \hspace{0.5em}SafeCoder & 24.50 & 29.63 & 17.07 \\
     \hspace{0.5em}\textbf{LPO-Reg} & 2.33 & 3.49 & 31.71 \\
     \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison with other security tuning methods.} FS and BL denote Function-Level and Block-Level security evaluations respectively. Pass@1 indicates the success rate of first attempt solutions.}
    \label{tab:security-tuning-comparison}
\end{table}

\subsection{Comaparison with Frontier Models}

\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l *{3}{c}}
     \toprule
     \multirow{3}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{Datasets}} \\
     \cmidrule(lr){2-4}
     & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX} \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
     & FS & BL & Pass@1 \\
     \midrule
     GPT-4o-mini & & & \\
     \hspace{0.5em}Basic & - & - & - \\
     \hspace{0.5em}Security Thinking & - & - & - \\
     GPT-4o & & &  \\
     \hspace{0.5em}Basic & - & - & - \\
     \hspace{0.5em}Security Thinking & - & - & - \\
     Claude-3.5-Sonnet & & & \\
     \hspace{0.5em}Basic & - & - & - \\
     \hspace{0.5em}Security Thinking & - & - & - \\
     \textbf{Best} & -- & -- & -- \\
     \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison with larger few-shot models.} FS and BL denote Function-Level and Block-Level security evaluations respectively.}
    \label{tab:large-model-comparison}
\end{table}

\subsection{Analysis}

\paragraph{Component Ablation}
\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l *{3}{c}}
     \toprule
     \multirow{3}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{Datasets}} \\
     \cmidrule(lr){2-4}
     & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX} \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
     & FS & BL & Pass@1 \\
     \midrule
     \textbf{CodeLlama} & -- & -- & -- \\
     \hspace{0.5em}\textit{w/o} synthetic data  & -- & -- & -- \\
     \hspace{0.5em}\textit{w/o} security thought  & -- & -- & -- \\
     \hspace{0.5em}\textit{w/o} regularization & -- & -- & -- \\
     \hspace{0.5em}full & -- & -- & -- \\
     \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation of different components of our methodology}:}
    \label{tab:security-tuning-comparison}
\end{table}

\paragraph{Error Analysis}


% \subsection{Comparison}

% \subsection{Comparison with Few-shot Prompting}

% \begin{table*}
%     \centering
%     \begin{tabular}{llllllllll}
%      \toprule
%      \multirow{3}{*}{Models} &\multirow{3}{*}{Types} & \multicolumn{8}{c}{Datasets}
%      \\
%      & & \multicolumn{2}{c}{SecEval} & \multicolumn{2}{c}{Asleep}  & \multicolumn{2}{c}{Synth.} & HumEval & MBPP
%      \\
%      \cmidrule(lr){3-4} 
%      \cmidrule(lr){5-6} 
%      \cmidrule(lr){7-8} 
%      \cmidrule(lr){9-9}
%      \cmidrule(lr){10-10}
%      & & FL & BL & FL & BL & FL & BL & Pass@1 & Pass@1
%      \\
%      \midrule
%      \multirow{5}{*}{Codellama} & Base & 50.77  & 80.77 & & & & & 25.61 &\\
%      & SFT  & 43.08  & 70.00 & & & & & 32.32 &\\
%      & PO  & 33.08  & 59.23 & & & & & 25.61 &\\
%      & LPO  & 28.46  & 43.85 & & & & & 26.22 &\\
%      & LPO-reg  & 43.08 & 73.08 & & & & & 31.1 &\\
%      \midrule
%      \multirow{5}{*}{Starcoder} & Base  & 45.38 & 76.92 & & & & & 27.44 &\\
%      & SFT  & 50.00 & 82.31 & & & & & 27.44 &\\
%      & PO  &  33.85 & 59.23 & & & & & 33.54 &\\
%      & LPO  & 20.77 & 30.77 & & & & & 25.0 &\\
%      & LPO-reg  &  40.77 & 80.77 & & & & &  25.0 &\\
%      \midrule
%      \multirow{5}{*}{Mistral} & Base  &  51.54 & 81.54 & & & & & 30.49 &\\
%      & SFT  &  44.62 & 73.85  & & & & & 42.07 &\\
%      & PO  & 30.00 & 52.31 & & & & & 31.71 &\\
%      & LPO  & 29.23 & 46.15 & & & & & 30.49 &\\
%      & LPO-reg  & 47.69 & 71.54 & & & & & 32.32 &\\
%      \midrule
%      \multirow{5}{*}{Phi2} & Base  &  50.77 & 76.92 & & & & & 46.34 &\\
%      & SFT  & 46.15 & 74.62 & & & & & 54.27 &\\
%      & PO  & 42.31 & 76.92 & & & & & 37.20 &\\
%      & LPO  & 44.62 & 69.23 & & & & & 47.56 &\\
%      & LPO-reg  & 46.15 & 72.31 & & & & & 53.05 &\\
%      \midrule
%     \end{tabular}
%     \caption{Code security performance of the various Code LLMs trained on our dataset.}
% \end{table*}



% \begin{table*}
%     \centering
%     \begin{tabular}{llllllllll}
%      \toprule
%      \multirow{3}{*}{Models} &\multirow{3}{*}{Types} & \multicolumn{8}{c}{Datasets}
%      \\
%      & & \multicolumn{2}{c}{SecEval} & \multicolumn{2}{c}{Asleep}  & \multicolumn{2}{c}{Synth.} & HumEval & MBPP
%      \\
%      \cmidrule(lr){3-4} 
%      \cmidrule(lr){5-6} 
%      \cmidrule(lr){7-8} 
%      \cmidrule(lr){9-9}
%      \cmidrule(lr){10-10}
%      & & FL & BL & FL & BL & FL & BL & Pass@1 & Pass@1
%      \\
%      \midrule
%      \multirow{5}{*}{Codellama} & Base & 53.72 & 80.17 & & & & & 28.05 &\\
%      & SFT  & 26.05 & 39.50 & & & & & 37.20 &\\
%      & PO  & 35.83 & 56.67 & & & & & 35.98 &\\
%      & LPO  & 12.77 & 20.21 & & & & & 27.44 &\\
%      & LPO-reg  & 21.85 & 30.25 & & & & & 30.49 &\\
%      \midrule
%      \multirow{5}{*}{Starcoder} & Base  & 58.12 & 88.03 & & & & & 32.93 &\\
%      & SFT  & 35.00 & 50.83 & & & & & 34.15 &\\
%      & PO  &  37.29 & 63.56& & & & & 37.2 &\\
%      & LPO  & 4.35 & 8.70  & & & & & 25.61 &\\
%      & LPO-reg  &  18.49 & 26.89 & & & & &  38.41 &\\
%      \midrule
%      \multirow{5}{*}{Mistral} & Base  &  55.83 & 83.33 & & & & & 27.44 &\\
%      & SFT  &  27.35 & 39.32 & & & & & 32.32 &\\
%      & PO  & 26.13 & 37.84 & & & & & 31.71 &\\
%      & LPO  & 11.97 & 22.22 & & & & & 32.93 &\\
%      & LPO-reg  & 8.85 & 9.73 & & & & & 31.1 &\\
%      \midrule
%      \multirow{5}{*}{Phi2} & Base  &  57.76 & 90.52 & & & & & 49.39 &\\
%      & SFT  & 29.06 & 40.17 & & & & & 53.66 &\\
%      & PO  & 30.77 & 40.17& & & & & 48.78 &\\
%      & LPO  & 14.02 & 17.76  & & & & & 50.0 &\\
%      & LPO-reg  & 17.95 & 25.64 & & & & & 48.78 &\\
%      \midrule
%     \end{tabular}
%     \caption{Code security performance of the various Code LLMs trained on our dataset.}
% \end{table*}



% \begin{table}
%     \centering
%     \begin{tabular}{llll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{3}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX}
%      \\
%      \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
%      & FS & BL & \multicolumn{1}{c}{Pass@1}
%      \\
%      \midrule
%      Phi-2
%      & &   
%      & 
%      \\
%      --SVEN
%      & 41.54 & 64.62
%      & 31.1
%      \\
%      --SafeCoder
%      & 20.00 & 27.69 
%      & 34.76
%      \\
%      --\textbf{Best}
%      &  &   
%      & 
%      \\
%      \midrule
%      Codellama
%      & &   
%      &
%      \\
%      --SafeCoder
%      &  &      
%      & 
%      \\
%      --\textbf{best}
%      &  &   
%      & 
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Comparison with other security tuning methods
%     }
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{llll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{3}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX}
%      \\
%      \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
%      & FS & BL & \multicolumn{1}{c}{Pass@1}
%      \\
%      \midrule
%      GPT-3.5 Turbo
%      & &   
%      & 
%      \\
%      GPT-4
%      &  & 
%      & 
%      \\
%      GPT-4o
%      & &     
%      & 
%      \\
%      \textbf{Best}
%      &  &   
%      & 
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Comparison with larger few-shot models
%     }
% \end{table}









% \begin{table*}
%     \centering
%     \begin{tabular}{lllllllllllll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{12}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{3}{c}{SecEval} & \multicolumn{3}{c}{LLMSecEval} & \multicolumn{3}{c}{PythonSecEval} & \multicolumn{3}{c}{Synthetic}
%      \\
%      \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
%      & FL & B & CQ & FL & B & CQ & FL & B & CQ & FL & B & CQ
%      \\
%      \midrule
%      Starcoder-1bn
%      & & &  
%      & & &
%      & & &
%      & & &
%      \\
%      --Base
%      & 51.54 & 52.38 & 40.00 
%      & & &
%      & & &
%      & & &
%      \\
%      --SFT
%      & 50.00 & 48.00 & 35.38   
%      & & &
%      & & &
%      & & &
%      \\
%      --PO
%      & 49.23 & 50.39 & 39.23 
%      & & &
%      & & &
%      \\
%      --LPO
%      & 50.77 & 51.18 & 39.23  
%      & & &
%      & & &
%      & & &
%      \\
%      \midrule
%      Phi-2-2.7bn
%      & & &  
%      & & &
%      & & &
%      & & &
%      \\
%      --Base
%      & 51.54 & 47.66 & 30.00 
%      & & &
%      & & &
%      & & &
%      \\
%      --SFT
%      & 49.23 & 51.20 & 30.77    
%      & & &
%      & & &
%      & & &
%      \\
%      --PO
%      & 14.62 & 16.15 & 0.00  
%      & & &
%      & & &
%      & & &
%      \\
%      --LPO
%      & 48.46 & 46.09 & 30.00    
%      & & &
%      & & &
%      & & &
%      \\
%      \midrule
%      CodeLlama-7bn
%      &  
%      & & &
%      & & &
%      & & &
%      \\
%      --Base
%      & 52.31 & 48.82 & 35.38 
%      & & &
%      & & &
%      & & &
%      \\
%      --SFT
%      & 49.23 & 49.61 & 34.62 
%      & & &
%      & & &
%      & & &
%      \\
%      --PO
%      & 46.15 & 46.40 & 24.62     
%      & & &
%      & & &
%      & & &
%      \\
%      --LPO
%      & 46.92 & 45.74 & 31.54    
%      & & &
%      & & &
%      & & &
%      \\
%      \midrule
%      Mistral-7bn
%      & & &  
%      & & &
%      & & &
%      & & &
%      \\
%      --Base
%      & 53.85 & 49.21 & 30.77 
 
%      & & &
%      & & &
%      & & &
%      \\
%      --SFT
%      & 48.46 & 47.29 & 32.31 
%      & & &
%      & & &
%      & & &
%      \\
%      --PO
%      & 43.85 & 45.38 & 30.77 
%      & & &
%      & & &
%      & & &
%      \\
%      --LPO
%      & 40.77 & 43.08 & 28.46  
%      & & &
%      & & &
%      & & &
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Code security performance of the various Code LLMs trained on our dataset.}
% \end{table*}


% \begin{table*}
%     \centering
%     \begin{tabular}{lllllllllll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{10}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{2}{c}{SecEval} & \multicolumn{2}{c}{LLMSec} & \multicolumn{2}{c}{PySec} & \multicolumn{2}{c}{Synth.}& \multicolumn{1}{c}{HumEval} & \multicolumn{1}{c}{MBPP}
%      \\
%      \cmidrule(lr){2-3} 
%      \cmidrule(lr){4-5} 
%      \cmidrule(lr){6-7} 
%      \cmidrule(lr){8-9}
%      \cmidrule(lr){10-10}
%      \cmidrule(lr){11-11}
%      & FS & BL & FS & BL & FS & BL & FS & BL & Pass@1 & Pass@1
%      \\
%      \midrule
%      Starcoder-1bn
%      & &   
%      & & 
%      & & 
%      & & 
%      &
%      &
%      \\
%      --Base
%      & 48.46 & 83.85
%      & & 
%      & & 
%      & & 
%      & 16.46
%      &
%      \\
%      --SFT
%      & 48.46 & 80.77
 
%      & & 
%      & & 
%      & & 
%      & 15.85
%      &
%      \\
%      --PO
%      & 0.00 & 0.00    
%      & & 
%      & & 
%      & & 
%      & 0
%      &
%      \\
%      --LPO
%      & 14.62 & 16.15    
%      & & 
%      & & 
%      & & 
%      & 0
%      &
%      \\
%      \midrule
%      Phi-2-2.7bn
%      & &   
%      & & 
%      & & 
%      & & 
%      &
%      &
%      \\
%      --Base
%      & 50.00 & 74.62
  
%      & & 
%      & & 
%      & & 
%      & 49.39
%      &
%      \\
%      --SFT
%      & 45.38 & 77.69
   
%      & & 
%      & & 
%      & & 
%      & 53.05
%      &
%      \\
%      --PO
%      & 0.00 & 0.00
   
%      & & 
%      & & 
%      & & 
%      & 0
%      &
%      \\
%      --LPO
%      & 14.62 & 16.15
   
%      & & 
%      & & 
%      & & 
%      & 0
%      &
%      \\
%      \midrule
%      CodeLlama-7bn
%      & &
%      & & 
%      & & 
%      & & 
%      &
%      &
%      \\
%      --Base
%      & 50.00 & 78.46   
%      & & 
%      & & 
%      & & 
%      & 29.88
%      &
%      \\
%      --SFT
%      & 47.69 & 83.85  
%      & & 
%      & & 
%      & & 
%      & 32.32
%      &
%      \\
%      --PO
%      & 44.62 & 70.00  
%      & & 
%      & & 
%      & & 
%      & 31.10
%      &
%      \\
%      --LPO
%      & 45.38 & 73.85   
%      & & 
%      & & 
%      & & 
%      & 25.61
%      &
%      \\
%      \midrule
%      Mistral-7bn
%      & &   
%      & & 
%      & & 
%      & & 
%      &
%      &
%      \\
%      --Base
%      & 50.77 & 74.62   
%      & & 
%      & & 
%      & & 
%      & 28.05
%      &
%      \\
%      --SFT
%      & 46.92 & 76.15   
%      & & 
%      & & 
%      & & 
%      & 28.05
%      &
%      \\
%      --PO
%      & 43.85 & 74.62   
%      & & 
%      & & 
%      & & 
%      & 29.88
%      &
%      \\
%      --LPO
%      & 34.62 & 56.92   
%      & & 
%      & & 
%      & & 
%      & 33.54
%      &
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Code security performance of the various Code LLMs trained on our dataset.}
% \end{table*}


% \begin{table}
%     \centering
%     \begin{tabular}{lll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{2}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{1}{c}{HumanEvalX} & \multicolumn{1}{c}{MBPP}
%      \\
%      \cmidrule(lr){2-2} \cmidrule(lr){3-3}
%      & \multicolumn{1}{c}{Pass@1} & \multicolumn{1}{c}{Pass@1}
%      \\
%      \midrule
%      Starcoder-1bn
%      & & 
%      \\
%      --Base
%      & 0 &
%      \\
%      --SFT
%      & 0 &
%      \\
%      --PO
%      & 0 &
%      \\
%      --LPO
%      & 0 &
%      \\
%      \midrule
%      Phi-2-2.7bn
%      & &
%      \\
%      --Base
%      & 47.56 &
%      \\
%      --SFT
%      & 54.88 &
%      \\
%      --PO
%      & 0 &
%      \\
%      --LPO
%      & 47.56 &
%      \\
%      \midrule
%      CodeLlama-7bn
%      & &
%      \\
%      --Base
%      & 29.88 &
%      \\
%      --SFT
%      & 32.93 &
%      \\
%      --PO
%      & 29.27&
%      \\
%      --LPO
%      & 26.22 & 
%      \\
%      \midrule
%      Mistral-7bn
%      & &
%      \\
%      --Base
%      & 25.61 &
%      \\
%      --SFT
%      & 28.05 & 
%      \\
%      --PO
%      & 29.27 & 
%      \\
%      --LPO
%      & 25.61 & 
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Code generation performance of the Code LLMs}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{lllll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{4}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{3}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX}
%      \\
%      \cmidrule(lr){2-4} \cmidrule(lr){5-5} 
%      & FL & B & CQ & \multicolumn{1}{c}{Pass@1}
%      \\
%      \midrule
%      Starcoder-1bn
%      & & &  
%      & 
%      \\
%      --SVEN
%      & 26.15 & 16.07 & 1.54  
%      & 0
%      \\
%      --SafeCoder
%      & 37.69 & 24.00 & 5.38 
%      & 0
%      \\
%      --LPO
%      & 50.77 & 51.18 & 39.23  
%      & 0
%      \\
%      \midrule
%      Phi-2-2.7bn
%      & & &  
%      & 
%      \\
%      --SVEN
%      & 52.31 & 45.69 & 26.92  
%      & 31.10
%      \\
%      --SafeCoder
%      & 35.38 & 21.62 & 8.46 
%      & 39.63
%      \\
%      --LPO
%      & 48.46 & 46.09 & 30.00
%      &  25.61
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Comparison with other security tuning methods
%     }
% \end{table}



% \begin{table*}
%     \centering
%     \begin{tabular}{llllllll}
%      \toprule
%      \multirow{3}{*}{Models} &\multirow{3}{*}{Types} & \multicolumn{6}{c}{Datasets}
%      \\
%      & & SecEval & LLMSec & Pysec & Synth. & HumEval & MBPP
%      \\
%      \cmidrule(lr){3-3} 
%      \cmidrule(lr){4-4} 
%      \cmidrule(lr){5-5} 
%      \cmidrule(lr){6-6}
%      \cmidrule(lr){7-7}
%      \cmidrule(lr){8-8}
%      & & Sec. & Sec. & Sec. & Sec. & Pass@1 & Pass@1
%      \\
%      \midrule
%      \multirow{5}{*}{Codellama-7B} & basic &  77.69 & & & & 28.05 &\\
%      & SFT & 53.08 & & & & 23.78 &\\
%      & PO &  78.46 & & & & 23.78 &\\
%      & LPO &  73.08 & & & & 23.78 &\\
%      & LPO-reg & 79.23 & & & & 24.39&\\
%      \midrule
%      \multirow{5}{*}{Starcoder-7B} & basic & 80.77& & & & 33.54&\\
%      & SFT &  76.15 & & & & 40.85 &\\
%      & PO & 38.46 & & & & 30.49 &\\
%      & LPO & 29.23 & & & & 30.49 &\\
%      & LPO-reg & 64.62 & & & & 31.71 &\\
%      \midrule
%      \multirow{5}{*}{Mistral-7B} & basic & 73.85 & & & & 28.05 &\\
%      & SFT & 73.08 & & & & 23.78 &\\
%      & PO &  73.85 & & & & 23.78 &\\
%      & LPO & 53.85 & & & & 23.78 &\\
%      & LPO-reg &  69.23 & & & & 24.39 &\\
%      \midrule
%      \multirow{5}{*}{Llama3-8B} & basic & 77.69 & & & & 55.49 &\\
%      & SFT &  75.38 & & & & 54.88 &\\
%      & PO &  77.69 & & & & 54.27 &\\
%      & LPO &  80.00 & & & & 50.00 &\\
%      & LPO-reg & 75.38 & & & & 53.05 &\\
%      \midrule
     
%      % \\
%      % \cmidrule(lr){2-3} 
%      % \cmidrule(lr){4-5} 
%      % \cmidrule(lr){6-7} 
%      % \cmidrule(lr){8-9}
%      % \cmidrule(lr){10-10}
%      % \cmidrule(lr){11-11}
%      % & FS & BL & FS & BL & FS & BL & FS & BL & Pass@1 & Pass@1
%      % \\
%      % \midrule
%      % Starcoder-1bn
%      % & &   
%      % & & 
%      % & & 
%      % & & 
%      % &
%      % &
%      % \\
%      % --Base
%      % & 48.46 & 83.85
%      % & & 
%      % & & 
%      % & & 
%      % & 16.46
%      % &
%      % \\
%      % --SFT
%      % & 48.46 & 80.77
 
%      % & & 
%      % & & 
%      % & & 
%      % & 15.85
%      % &
%      % \\
%      % --PO
%      % & 0.00 & 0.00    
%      % & & 
%      % & & 
%      % & & 
%      % & 0
%      % &
%      % \\
%      % --LPO
%      % & 14.62 & 16.15    
%      % & & 
%      % & & 
%      % & & 
%      % & 0
%      % &
%      % \\
%      % \midrule
%      % Phi-2-2.7bn
%      % & &   
%      % & & 
%      % & & 
%      % & & 
%      % &
%      % &
%      % \\
%      % --Base
%      % & 50.00 & 74.62
  
%      % & & 
%      % & & 
%      % & & 
%      % & 49.39
%      % &
%      % \\
%      % --SFT
%      % & 45.38 & 77.69
   
%      % & & 
%      % & & 
%      % & & 
%      % & 53.05
%      % &
%      % \\
%      % --PO
%      % & 0.00 & 0.00
   
%      % & & 
%      % & & 
%      % & & 
%      % & 0
%      % &
%      % \\
%      % --LPO
%      % & 14.62 & 16.15
   
%      % & & 
%      % & & 
%      % & & 
%      % & 0
%      % &
%      % \\
%      % \midrule
%      % CodeLlama-7bn
%      % & &
%      % & & 
%      % & & 
%      % & & 
%      % &
%      % &
%      % \\
%      % --Base
%      % & 50.00 & 78.46   
%      % & & 
%      % & & 
%      % & & 
%      % & 29.88
%      % &
%      % \\
%      % --SFT
%      % & 47.69 & 83.85  
%      % & & 
%      % & & 
%      % & & 
%      % & 32.32
%      % &
%      % \\
%      % --PO
%      % & 44.62 & 70.00  
%      % & & 
%      % & & 
%      % & & 
%      % & 31.10
%      % &
%      % \\
%      % --LPO
%      % & 45.38 & 73.85   
%      % & & 
%      % & & 
%      % & & 
%      % & 25.61
%      % &
%      % \\
%      % \midrule
%      % Mistral-7bn
%      % & &   
%      % & & 
%      % & & 
%      % & & 
%      % &
%      % &
%      % \\
%      % --Base
%      % & 50.77 & 74.62   
%      % & & 
%      % & & 
%      % & & 
%      % & 28.05
%      % &
%      % \\
%      % --SFT
%      % & 46.92 & 76.15   
%      % & & 
%      % & & 
%      % & & 
%      % & 28.05
%      % &
%      % \\
%      % --PO
%      % & 43.85 & 74.62   
%      % & & 
%      % & & 
%      % & & 
%      % & 29.88
%      % &
%      % \\
%      % --LPO
%      % & 34.62 & 56.92   
%      % & & 
%      % & & 
%      % & & 
%      % & 33.54
%      % &
%      % \\
%      % \bottomrule
%     \end{tabular}
%     % \caption{Code security performance of the various Code LLMs trained on our dataset.}
% \end{table*}









% \begin{table}
%     \centering
%     \begin{tabular}{llll}
%      \toprule
%      \multirow{3}{*}{Models} & \multicolumn{3}{c}{Datasets}
%      % A & B & C & D & E
%      \\
%      & \multicolumn{2}{c}{SecEval} & \multicolumn{1}{c}{HumanEvalX}
%      \\
%      \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
%      & FS & BL & \multicolumn{1}{c}{Pass@1}
%      \\
%      \midrule
%      Starcoder-1bn
%      & &   
%      & 
%      \\
%      --SVEN
%      &  & 
%      & 
%      \\
%      --SafeCoder
%      & &     
%      & 
%      \\
%      --LPO
%      &  &   
%      & 0
%      \\
%      \midrule
%      Phi-2-2.7bn
%      & &   
%      &
%      \\
%      --SVEN
%      &  & 

%      & 
%      \\
%      --SafeCoder
%      &  &      
%      & 
%      \\
%      --LPO
%      &  &   
%      & 
%      \\
%      \bottomrule
%     \end{tabular}
%     \caption{Comparison with other security tuning methods
%     }
% \end{table}








% \begin{table*}
% \begin{subtable}{0.5\linewidth}
% \small
% \centering
% \begin{tabular}{l*{8}{c}}  % Center-align numeric columns
%      \toprule
%      \multirow{3}{*}{\textbf{Models}} & \multicolumn{8}{c}{\textbf{Datasets}} \\
%      \cmidrule(lr){2-9}
%      & \multicolumn{2}{c}{SecEval} & \multicolumn{2}{c}{Asleep} & \multicolumn{2}{c}{LLMSec} & \multicolumn{2}{c}{Synth.}\\
%      \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%      & \texttt{CS} & \texttt{EnB} & \texttt{CS} & \texttt{EnB} & \texttt{CS} & \texttt{EnB} & \texttt{CS} & \texttt{EnB}\\
%      \midrule
%     \textbf{CodeLlama-7b}  
%     & 46.0 & 0.84
%     & 0.0 & 4.68
%     & 52.3 & 1.02
%     & 64.3 & 0.83
%     \\
%     -- \texttt{It}
%     & 81.2 & 0.31
%     & 10.8 & 1.45   
%     & 59.7 & 0.62
%     & 80.2 & 0.31
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 70.8 & 0.47  
%     & 10.0 & 1.52  
%     & 61.2 & 0.64 
%     & 80.6 & 0.30 
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 85.3 & 0.27    
%     & 48.8 & 0.71  
%     & 77.7 & 0.35   
%     & 87.7 & 0.20 
%     \\
%      \midrule
%      \textbf{Starcoder2-7b}  
%     & 44.2 & 0.87 
%     & 0.0 & 4.98  
%     & 32.7 & 2.20
%     & 57.4 & 1.00
%     \\
%     -- \texttt{It}
%     & 72.9 & 0.45
%     & 7.8 & 1.88
%     & 63.1 & 0.70  
%     & 83.3 & 0.28
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 73.9 & 0.41   
%     & 5.3 & 1.85   
%     & 58.9 & 0.78 
%     & 83.0 & 0.27
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 83.6 & 0.22   
%     & 24.4 & 1.61   
%     & 77.8 & 0.32 
%     & 81.8 & 0.30  
%     \\
%     \midrule
%     \textbf{Mistral-7b}  
%     & 47.0 & 0.84
%     & 0.0 & 4.03 
%     & 29.8 & 1.78 
%     & 55.1 & 0.84
%     \\
%     -- \texttt{It}
%     & 72.0 & 0.39
%     & 10.8 & 1.63 
%     & 61.0 & 0.57  
%     & 79.1 & 0.33  
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 94.1 & 0.09
%     & 83.9 & 0.29   
%     & 93.2 & 0.11
%     & 95.8 & 0.06 
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 97.7 & 0.03   
%     & 85.8 & 0.30   
%     & 96.8 & 0.04   
%     & 97.6 & 0.04 
%     \\
%     \midrule
%     \textbf{Phi-2-2.7b}  
%     & 47.5 & 0.88 
%     & 0.0 & 4.21 
%     & 23.0 & 1.68
%     & 56.0 & 0.84 
%     \\
%     -- \texttt{It}
%     & 76.6 & 0.33 
%     & 23.8 & 1.26  
%     & 69.2 & 0.49  
%     & 80.1 & 0.32
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 75.2 & 0.35  
%     & 20.7 & 1.32  
%     & 72.4 & 0.48  
%     & 81.5 & 0.30 
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 80.8 & 0.28    
%     & 19.2 & 1.48   
%     & 74.0 & 0.45   
%     & 83.1 & 0.29   
%     \\
%      \bottomrule
%     \end{tabular}
%     \caption{\textbf{Security performance of \name}:}
%     \label{tab:security_performance}

% \end{subtable}

% \begin{subtable}{0.5\linewidth}
% \small
% \centering
% \begin{tabular}{l*{2}{c}}  % Center-align numeric columns
%      \toprule
%      \multirow{3}{*}{\textbf{Models}} & \multicolumn{2}{c}{\textbf{Datasets}} \\
%      \cmidrule(lr){2-3}
%      & HumanEvalX & MBXP\\
%      \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
%      & \texttt{Pass@1} & \texttt{Pass@1}\\
%      \midrule
%     \textbf{CodeLlama-7b}  
%     & 29.3
%     & 45.8
%     \\
%     -- \texttt{It}
%     & 36.6 
%     & 48.5
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 34.1
%     & 48.1
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 36.6  
%     & 49.6
%     \\
%      \midrule
%      \textbf{Starcoder2-7b}  
%     & 31.7
%     & 50.0
%     \\
%     -- \texttt{It}
%     & 39.0
%     & 56.5
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 40.2
%     & 55.8
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 40.9 
%     & 53.5
%     \\
%     \midrule
%     \textbf{Mistral-7b}  
%     & 24.4 
%     & 37.3
%     \\
%     -- \texttt{It}
%     & 37.8
%     & 50.0
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 37.8
%     & 50.0
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 31.7  
%     & 50.0
%     \\
%     \midrule
%     \textbf{Phi-2-2.7b}  
%     & 50.0 
%     & 45.4
%     \\
%     -- \texttt{It}
%     & 53.0
%     & 56.5
%     \\
%     -- \texttt{It} + \texttt{PO}
%     & 53.7 
%     & 56.9
%     \\
%     -- \texttt{It} + \texttt{LPO-Reg}
%     & 53.0  
%     & 58.9  
%     \\
%      \bottomrule
%     \end{tabular}
%     \caption{\textbf{Security performance of \name}:}
%     \label{tab:security_performance}

% \end{subtable} 
% \caption{}
% \end{table*}


